Nonlinear Controllability Assessment of Aerial Manipulator Systems using Lagrangian Reduction

This paper analyzes the nonlinear Small-Time Local Controllability (STLC) of a class of underatuated aerial manipulator robots. We apply methods of Lagrangian reduction to obtain their lowest dimensional equations of motion (EOM). The symmetry-breaking potential energy terms are resolved using advected parameters, allowing full $SE(3)$ reduction at the cost of additional advection equations. The reduced EOM highlights the shifting center of gravity due to manipulation and is readily in control-affine form, simplifying the nonlinear controllability analysis. Using Sussmann's sufficient condition, we conclude that the aerial manipulator robots are STLC near equilibrium condition, requiring Lie bracket motions up to degree three.

==> AppA.tex <==
Based on the working mechanism of the rotor, the rotational velocity of the $j^{th}$ rotor in the $B$ frame $\omega_{r_j}^b$ is $\Omega_je_3$ since we assume $z_{R_j}$ for all $j$ and $z_{B}$ are parallel unit vectors pointing in the same direction. Therefore, the rotational velocity of the $j^{th}$ rotor with respect to $r_j$ is:
\begin{equation}
    \omega_{r_j} = R_{r_jb}\omega_b + R_{r_jb}\Omega_je_3
\end{equation}
Then, the rotational kinetic energy of the $j^{th}$ rotor is:
\small
\begin{equation} \label{eq:rotKE_jthrotor}
    \begin{array}{lll}
    K_{r_j,r} = \frac{1}{2}\left< \omega_{r_j}, I_r \omega_{r_j}  \right>
    = \frac{1}{2}\left< R_{r_jb}\omega_b , I_rR_{r_jb} \omega_b   \right> \\ + \left< R_{r_jb}\omega_b , I_r R_{r_jb} e_{3} \right>\Omega_j  +  \frac{1}{2}\left< R_{r_jb}e_3 , I_rR_{r_jb} e_{3}\right> \left(\Omega_j \right)^2
     \end{array}
\end{equation}
\normalsize
Since the rotors are modelled as a rotating symmetric cylinder and the $z$ axis among $R_j$ and $B$ frames are equivalent, we can make the following simplification $R_{r_jb}^T I_r R_{r_jb} =  I_{r}$, $\left< R_{r_jb}e_3 , I_rR_{r_jb} e_{3}\right> = J$, and $\left< R_{r_jb}\omega_b , I_r R_{r_jb} e_{3} \right> = Je_3^T \omega_b$. Substituting these property, Eq. \ref{eq:rotKE_jthrotor} can be simplified to Eq. \ref{eq:rotor_rotationalKE}. Alternative derivations uses mass flow integrated over the volume of the rotor cylinder as:
\begin{equation}
    K_{R_j,r} = \frac{1}{2}\int_{V}\rho(r) \|(\omega_b \times R_{r_jb} + \dot{R}_{r_jb})r \|_2^2\, dV.
\end{equation}
This method also produces the same result, and the details will be omitted. 


==> AppB.tex <==
The mass matrix $\mathcal{M}(q)$ is conveniently partitioned as Eq. $\ref{eq:mass_part}$ which can be further partition and computed as the following:\\
\begin{equation}
\mathcal{M} =  \left[\begin{array}{cc|c|cc}
          \mathcal{M}_{11} & \mathcal{M}_{12}& \mathcal{M}_{13}& \mathcal{M}_{14}& \mathcal{M}_{15}\\
          \mathcal{M}_{12}^{T} & \mathcal{M}_{22}& \mathcal{M}_{23}& \mathcal{M}_{24}& \mathcal{M}_{25}\\\hline
          \mathcal{M}_{13}^{T} & \mathcal{M}_{23}^{T}& \mathcal{M}_{r}& \mathcal{M}_{34}& \mathcal{M}_{35}\\\hline
          \mathcal{M}_{14}^{T} & \mathcal{M}_{24}^{T}& \mathcal{M}_{34}^{T}& \mathcal{M}_{44}& \mathcal{M}_{45}\\
           \mathcal{M}_{15}^{T} & \mathcal{M}_{25}^{T}& \mathcal{M}_{35}^{T}& \mathcal{M}_{45}^{T}& \mathcal{M}_{55}\\
\end{array} \right]
\end{equation}
where\\
\small
$$
\begin{array}{ll}
    \mathcal{M}_{11} &= (m_1+m_2+m_s+2nm_r)I_{3\times 3}\in\mathbb{R}^{3\times 3}\\
    \mathcal{M}_{12} &= -m_1S(g_{bl_1}(\eta_1))-m_2S(g_{bl_2}(\eta_1,\eta_2))\in\mathbb{R}^{3\times 3}\\
    \mathcal{M}_{13} &= 0_{3\times 2n} \in\mathbb{R}^{3\times 2n}\\
    \mathcal{M}_{14} &= m_1J_{l,bl_{1}}^{b}(\eta_1) + m_2J_{l,bl_{2}}^{b}(\eta_1,\eta_2)\left[\begin{array}{c}
         1\\
         0
    \end{array} \right] \in\mathbb{R}^{3\times 1}\\
    \mathcal{M}_{15} &= m_2J_{l,bl_{2}}^{b}(\eta_1,\eta_2)\left[\begin{array}{c}
        0\\
         1
    \end{array} \right] \in\mathbb{R}^{3\times 1}\\
    \mathcal{M}_{22} &= I_{b}+2n(I_{r}-\sigma^{2}m_r)+R_{bl_1}I_1R_{bl_1}^{T}+R_{bl_1}R_{l_1l_2}I_2R_{l_1l_2}^{T}R_{bl_1}^{T} \\&+m_{1}S\left(g_{bl_1}(\eta_1)\right)^{T}S(g_{bl_1}(\eta_1))\\&+m_{2}S\left(g_{bl_2}(\eta_1,\eta_2)\right)^{T}S(g_{bl_2}(\eta_1,\eta_2)) \in\mathbb{R}^{3\times 3}\\
    \mathcal{M}_{23} &= Je_{3}\mathbf{1}_{1\times 2n} \in\mathbb{R}^{3\times 2n}\\
    \mathcal{M}_{24} &= R_{bl_1}I_1R_{bl_1}^{T}\left(J_{r,bl_1}^{b}\right)+R_{bl_1}R_{l_1l_2}I_2R_{l_1l_2}^{T}R_{bl_1}^{T}\left(J_{r,bl_2}^{b}\right)\left[\begin{array}{c}
        1\\
        0
    \end{array} \right]\\&-m_1S\left(g_{bl_1}(\eta_1)\right)^{T}J_{l,bl_1}^{b}\\&-m_2S\left(g_{bl_2}(\eta_1,\eta_2)\right)^{T}J_{l,bl_{2}}^{b}(\eta_1,\eta_2)\left[\begin{array}{c}
         1\\
         0
    \end{array} \right]\in\mathbb{R}^{3\times 1}
\end{array}
$$

$$\begin{array}{ll}
    \mathcal{M}_{25} &= R_{bl_1}R_{l_1l_2}I_2R_{l_1l_2}^{T}R_{bl_1}^{T}\left(J_{r,bl_2}^{b}\right)\left[\begin{array}{c}
        0\\
        1
    \end{array} \right]\\& -m_2S\left(g_{bl_2}(\eta_1,\eta_2)\right)^{T}J_{l,bl_{2}}^{b}(\eta_1,\eta_2)\left[\begin{array}{c}
         0\\
         1
    \end{array} \right]\in\mathbb{R}^{3\times 1}\\
    \mathcal{M}_{r} &= JI_{2n\times 2n} \in \mathbb{R}^{2n\times 2n} \\
    \mathcal{M}_{34} &= 0_{2n\times 1} \in \mathbb{R}^{2n\times 1} \\
    \mathcal{M}_{35} &= 0_{2n\times 1} \in \mathbb{R}^{2n\times 1} \\
    \mathcal{M}_{44} &= \left(J_{r,bl_1}^{b}\right)^{T}R_{bl_1}I_1R_{bl_1}^{T}\left(J_{r,bl_2}^{b}\right)+m_1\left( J_{l,bl_{1}}^{b}(\eta_1)\right)^{T}J_{l,bl_{1}}^{b}(\eta_1)\\&+\left[\begin{array}{c}
        1\\
        0
    \end{array} \right]^{T}\left(J_{r,bl_2}^{b}\right)^{T}R_{bl_1}R_{l_1l_2}I_2R_{l_1l_2}^{T}R_{bl_1}^{T}\left(J_{r,bl_1}^{b}\right)\left[\begin{array}{c}
        1\\
        0
    \end{array} \right]\\& +m_2\left[\begin{array}{c}
        1\\
        0
    \end{array} \right]^{T}\left( J_{l,bl_{2}}^{b}(\eta_1,\eta_2)\right)^{T}J_{l,bl_{2}}^{b}(\eta_1,\eta_2)\left[\begin{array}{c}
        1\\
        0
    \end{array} \right] \in\mathbb{R}
\end{array}
$$

$$
\begin{array}{ll}
    \mathcal{M}_{45} &=  m_2\left[\begin{array}{c}
         1\\
         0
    \end{array} \right]^{T}\left(J_{l,bl_{2}}^{b}(\eta_1,\eta_2) \right)^{T}\left(J_{l,bl_{2}}^{b}(\eta_1,\eta_2) \right)\left[\begin{array}{c}
         0\\
         1
    \end{array} \right]\\&+ \left[\begin{array}{c}
        1\\
        0
    \end{array} \right]^{T}\left(J_{r,bl_2}^{b}\right)^{T}R_{bl_1}R_{l_1l_2}I_2R_{l_1l_2}^{T}R_{bl_1}^{T}\left(J_{r,bl_1}^{b}\right)\left[\begin{array}{c}
        0\\
        1
    \end{array} \right] \in\mathbb{R}\\
    \mathcal{M}_{55} &= \left[\begin{array}{c}
        0\\
        1
    \end{array} \right]^{T}\left(J_{r,bl_2}^{b}\right)^{T}R_{bl_1}R_{l_1l_2}I_2R_{l_1l_2}^{T}R_{bl_1}^{T}\left(J_{r,bl_1}^{b}\right)\left[\begin{array}{c}
        0\\
        1
    \end{array} \right] \\&+ m_2\left[\begin{array}{c}
         0\\
         1
    \end{array} \right]^{T}\left(J_{l,bl_{2}}^{b}(\eta_1,\eta_2) \right)^{T}\left(J_{l,bl_{2}}^{b}(\eta_1,\eta_2) \right)\left[\begin{array}{c}
         0\\
         1
    \end{array} \right]\in\mathbb{R}\\
\end{array}
$$
\normalsize

==> STLC.tex <==
\begin{thm}
Any aerial manipulator system satisfies the definition of AM is small-time locally controllable (STLC) evaluated at the equilibrium conditions, eq. \ref{eq:eqlib_c1} - \ref{eq:eqlib_c4}, except for the manipulator singularity at $[\eta_1,\eta_2]= [\pi/2,0]$.
\begin{pf}  
By definition of good and bad brackets, all Lie brackets used to establish STLA are classified as good brackets. The highest degree bracket used to span $T_{\mathbf{q}}Q$ is \textbf{four}. To apply theorem \ref{thm: sussmann}, we need to show all bad brackets of degree $j\leq 4$ can be expressed as a linear combination of god brackets of degree less than $j$. By the definition of bad brackets, there will be no bad brackets associated with an even degree. Then, the bad brackets of the third degree can be expressed generally as $[[f,g_i],g_i],\forall i\in \{1,\cdots,2n+2\}$. More specifically, for $i \in \{1,2\}$ the bad brackets evaluated at the equilibrium condition takes the following form:
\small
\begin{equation}
     [[f,g_{i}],g_i]\big|_{\mathbf{q}=\mathbf{q}^*} =\left[\begin{array}{cccc} 
         0^{[\dot{p}_{b},\dot{\mathbf{\Theta}},\dot{\mathbf{p}},\dot{\mathbf{l}}]}_{1\times 12}& 0^{\dot{\eta}}_{1\times 2}&  f^{\ddot{\eta}}_{1\times 2}(\eta)&         0^{\mathbf{\dot{\Omega}}}_{1\times 2n}
     \end{array} \right],
\end{equation}
\normalsize
which can be annihilated with good, degree 1 bracket $g_1$ and $g_2$. The remaining $2n$ third degree bad brackets take the general form:
\small
\begin{equation}
\begin{array}{ll}
   [[f,g_{i}],g_i]\big|_{\mathbf{q}=\mathbf{q}^*} =  \left[\begin{array}{c} \left[\begin{array}{ccc}
     0^{\dot{p}_{b_x}} &  f^{\dot{p}_{b_y}}(\eta) & 0^{\dot{p}_{b_z}}
   \end{array}\right]^{T} \\
   \left[\begin{array}{ccc}
     f^{\dot{\phi}} &  0^{\dot{\theta}} & f^{\dot{\psi}}
   \end{array}\right]^{T} \\
    \left[\begin{array}{ccc}
     0^{\dot{\mathbf{p}}_x} &  0^{\dot{\mathbf{p}}_y} & f^{\dot{\mathbf{p}}_z}
   \end{array}\right]^{T} \\
   f^{\dot{\mathbf{l}}}_{3\times1} \\ 0^{[\dot{\eta},\ddot{\eta},\dot{\mathbf{\Omega}}]}_{2n+4 \times 1}
    \end{array}\right]
\end{array} 
\end{equation} 
\normalsize
which can be expressed as a linear combinations of the following brackets:
\begin{equation}
    [f,g_3],\cdots,[f,g_{2n+2}],[[f,g_3],f],\cdots,[[f,g_{2n+2}],f]
\end{equation}
The final bad bracket is the drift term evaluated at equilibrium conditions. Since by the definition of equilibrium condition, we have $\dot{\mathbf{q}}^* =  f(\mathbf{q}^*) + G(\mathbf{q}^*)\mathbf{u^*}= 0$. Equivalently, the first order bad bracket $f$ can be expressed as
\begin{equation}
   f(\mathbf{q}^*) =  -\sum_{i=1}^{2n+2} g_{i}(\mathbf{q}^*)\mathbf{u^*},
\end{equation}
a linear combination of the first order good brackets $g_{i},\forall i\in {1,\cdots,2n+2}$.  Thus, all bad brackets of degree $k\leq 4$ can be written as combinations of good Lie brackets of degree $j\leq k$. By Sussmann's condition \ref{thm: sussmann}, STLC is establish for the defined aerial manipulator class at the equilibrium conditions \ref{eq:eqlib_c1} - \ref{eq:eqlib_c4} except for the manipulator singularity at $[\eta_1,\eta_2]= [\pi/2,0]$.
\end{pf}
Despite we can formally prove that AM systems are STLA and STLC, both conditions are binary results and insufficient to be a solely design criteria for any system. As briefly mentioned, the higher order brackets are much "slower" in comparison with the lower order ones. If the system is highly unstable or have uncertainties in modeling, a system with STLC could still be uncontrollable in real world application. To improve our STLC result, we would like to develop an alternative metric that evaluates the "degree of controllability" of a given system. Further, link the system dynamics with the degree of controllability as a new design criteria for mechanical systems.\\
On the other hand, to use Sussmann's condition, the rate of change of rotor RPM was introduced as an alternative control input which is bilateral. Realistically speaking, the negative rate of changes of rotor RPM are much harder to generate and couples with resistive torques, one of the more under-explored territory due to its coupling with aerial dynamic damping and the motor's electromotive force. Therefore, it will be rewarding there are less restrictive conditions for underactuated system with unilateral control inputs as the result by \cite{goodwineUCI}.  
\end{thm}

